An Efficient Data Reuse with Tile-Based Adaptive Stationary for Transformer Accelerators

Transformer-based models have become the \textit{de facto} backbone across many fields, such as computer vision and natural language processing. However, as these models scale in size, external memory access (EMA) for weight and activations becomes a critical bottleneck due to its significantly higher energy consumption compared to internal computations. While most prior work has focused on optimizing the self-attention mechanism, little attention has been given to optimizing data transfer during linear projections, where EMA costs are equally important. In this paper, we propose the Tile-based Adaptive Stationary (TAS) scheme that selects the input or weight stationary in a tile granularity, based on the input sequence length. Our experimental results demonstrate that TAS can significantly reduce EMA by more than 97\% compared to traditional stationary schemes, while being compatible with various attention optimization techniques and hardware accelerators.

==> Makefile <==
TARGET=main
LATEX_BUILD_CMD=xelatex -synctex=1 -shell-escape -interaction=nonstopmode

default: build

build:
	$(LATEX_BUILD_CMD) $(TARGET).tex
	bibtex main.aux || true
	$(LATEX_BUILD_CMD) $(TARGET).tex
	$(LATEX_BUILD_CMD) $(TARGET).tex | grep 'Warning\|pages'
clean:
	rm -rf *.aux *.log *.gz *.bbl *.blg *.lof *.lot *.toc *.out


==> ack/ack.tex <==
\begin{acknowledgement}%
在這兩年的碩士生涯中，我學到了如何探索並研究專業領域的知識，也使自己在面對問題時的思維更清晰。實驗室的生活讓我學到如何與他人合作並運用所學來達成目標。

首先，我要感謝我的指導教授張添烜老師，在我還是大學部專題生時，帶領沒有程式、沒有系統基礎的我，一步一步認識了數位電路設計、神經網路演算法的領域，在進入研究所後，不僅在研究上給予充足的資源，也給予了我高度的自由，而且即使在百忙之中，還是無時無刻的提供我一些建議與想法，讓我在研究中不會迷失方向，順利地進行研究與發表論文。另外，我也要感謝陳巍仁、侯拓宏、周世傑、陳宏明、劉建男教授，在每個週的計畫聯合會議中，總是會給我一些意見或是可以改進的建議，使我的研究更加充實，讓我思考的面向能夠更全面，透過計畫合作讓我學習到數位電路與深度學習以外領域的知識。

大三時，我修習了老師開的數位電路與系統這門課，很感謝當時的助教子翾、建德、國威三位學長積極、耐心且風趣的指導，協助我初學數位電路時快速上手並讓我下定決心走數位電路設計這條路，並且三位學長也作為我心中助教的模範，深深影響我往後擔任助教時的教學風格。再來感謝實驗室的研究夥伴們，讓我在辛苦的碩士期間多了許多歡樂，也在研究以外得到許多幫助。感謝易群、國威、建德、宇翔、家碩、云涓學長姊們的教導與建議。感謝敦皓、仲緯、啟豪、立維、鈺涵一同陪伴度過最艱難的時刻，也和你們共度了一段快樂的時光。感謝晏誠、子嘉、姚遠、志嘉、蔣洛亘、洪毅的協助與支持。感謝相同研究計畫團隊的力愷、士航，在研究上一起討論問題、解決困難也給予了我許多幫助，沒有你們不會有今天的我。感謝電子實驗的王夢偉、陳建安助教、學長昱賢和助教夥伴邵宇、均承、庭惠，除了給予我許多人生建議也陪伴我度過很多歡樂時光。

最後，我要感謝我的母親，總是無條件支持並鼓勵我的任何決定，讓我可以無後顧之憂地完成學業，還有感謝我的姊姊，希望我沒有辜負妳對我的期待。

\end{acknowledgement}


==> thesis_new.tex <==
\ProvidesClass{thesis}[2022/02/25 V2.0]
\NeedsTeXFormat{LaTeX2e}


\DeclareOption*{\PassOptionsToClass{\CurrentOption}{book}}

\newif\ifTHESISOPTIONmaster         \THESISOPTIONmastertrue
\newif\ifTHESISOPTIONphd            \THESISOPTIONphdfalse

\DeclareOption{master}{\THESISOPTIONmastertrue\THESISOPTIONphdfalse}
\DeclareOption{phd}{\THESISOPTIONmasterfalse\THESISOPTIONphdtrue}

\newif\ifTHESISOPTIONen             \THESISOPTIONentrue
\newif\ifTHESISOPTIONzh             \THESISOPTIONzhfalse

\DeclareOption{en}{\THESISOPTIONentrue\THESISOPTIONzhfalse}
\DeclareOption{zh}{\THESISOPTIONenfalse\THESISOPTIONzhtrue}

\newif\ifTHESISOPTIONbinding      \THESISOPTIONbindingfalse
\DeclareOption{binding}{\THESISOPTIONbindingtrue}

\newif\ifTHESISOPTIONreview         \THESISOPTIONreviewfalse
\newif\ifTHESISOPTIONdraft          \THESISOPTIONdrafttrue
\newif\ifTHESISOPTIONfinal          \THESISOPTIONfinalfalse

\DeclareOption{review}{\THESISOPTIONreviewtrue
                       \THESISOPTIONdraftfalse
                       \THESISOPTIONfinalfalse
                       \THESISOPTIONbindingfalse}

\DeclareOption{draft}{\THESISOPTIONreviewfalse
                      \THESISOPTIONdrafttrue
                      \THESISOPTIONfinalfalse
                      \THESISOPTIONbindingfalse}

\DeclareOption{final}{\THESISOPTIONreviewfalse
                      \THESISOPTIONdraftfalse
                      \THESISOPTIONfinaltrue
                      \THESISOPTIONbindingtrue}

\newif\ifTHESISOPTIONwatermark      \THESISOPTIONwatermarkfalse
\DeclareOption{watermark}{\THESISOPTIONwatermarktrue}

\ProcessOptions
\LoadClass[a4paper,12pt,oneside]{book}


\usepackage[BoldFont, SlantFont, CJKchecksingle, CJKmath=true]{xeCJK}
\usepackage{fontspec}     %
\usepackage{ifplatform}   %
\usepackage{indentfirst}  %
\usepackage{setspace}     %
\usepackage{tikz}         %
\usepackage{eso-pic}      %
\usepackage[xetex, hidelinks]{hyperref}  %
\usepackage{geometry}     %
\usepackage{emptypage}    %
\usepackage{afterpage}    %
\usepackage{lipsum}       %
\usepackage{verbatim}     %
\usepackage[retainorgcmds]{IEEEtrantools}  %
\usepackage{xCJKnumb}     %
\usepackage{titlesec}     %
\usepackage{titletoc}     %
\usepackage{tocloft}	  %
\usepackage{caption}	  %
\usepackage[labelformat=simple]{subcaption} %
\usepackage[chapter]{algorithm}  %


\ifTHESISOPTIONbinding  %
  \geometry{left=3 cm, right=2 cm, top=3 cm, bottom=3 cm}%
\else
  \geometry{left=2.5 cm, right=2.5 cm, top=3 cm, bottom=3 cm}%
\fi

\pagestyle{plain}
\setlength{\footskip}{1.5cm}

\doublespacing


\newcommand{\mainfont}[1]{%
\ifx&#1&%
  \setmainfont[Ligatures=TeX]{Times New Roman}
\else
  \setmainfont[Ligatures=TeX]{#1}
\fi
}

\newcommand{\sansfont}[1]{%
\ifx&#1&%
  \setsansfont[Ligatures=TeX]{Arial}
\else
  \setsansfont[Ligatures=TeX]{#1}
\fi
}


\newcommand{\mainfontzh}[1]{%
\ifx&#1&%
  \ifwindows  %
    \setCJKmainfont{DFKai-SB}  %
  \else\iflinux  %
    \setCJKmainfont{AR PL UKai TW}  %
  \else\ifmacosx  %
    \setCJKmainfont{Kaiti TC Regular}  %
  \else  %
    \setCJKmainfont{DFKai-SB}
  \fi\fi\fi
\else
  \setCJKmainfont{#1}
\fi
}

\newcommand{\sansfontzh}[1]{%
\ifx&#1&%
  \ifwindows  %
    \setCJKsansfont{PMingLiU}  %
  \else\iflinux  %
    \setCJKsansfont{AR PL UMing TW}  %
  \else\ifmacosx  %
    \setCJKsansfont{LiSong Pro}  %
  \else  %
    \setCJKsansfont{PMingLiU}
  \fi\fi\fi
\else
  \setCJKsansfont{#1}
\fi
}

\XeTeXlinebreaklocale "zh"
\XeTeXlinebreakskip = 0pt plus 1pt


\def\titlezh#1{\gdef\@titlezh{#1}}

\def\degreeyear#1{\gdef\@degreeyear{#1}}
\def\degreemonth#1{\gdef\@degreemonth{#1}}

\def\degreeyearzh#1{\gdef\@degreeyearzh{#1}}

\def\nation#1{\gdef\@nation{#1}}

\def\yearmonth#1{\gdef\@yearmonth{#1}}

\def\degree#1{\gdef\@degree{#1}}

\def\field#1{\gdef\@field{#1}}

\def\thesistype#1{\gdef\@thesistype{#1}}

\def\thesistypezh#1{\gdef\@thesistypezh{#1}}

\def\institute#1{\gdef\@institute{#1}}

\def\institutezh#1{\gdef\@institutezh{#1}}

\def\college#1{\gdef\@college{#1}}

\def\university#1{\gdef\@university{#1}}

\def\universityzh#1{\gdef\@universityzh{#1}}

\def\location#1{\gdef\@location{#1}}

\def\advisor#1{\gdef\@advisor{#1}}

\def\advisorzh#1{\gdef\@advisorzh{#1}}

\def\coadvisorA#1{\gdef\@coadvisorA{#1}}

\def\coadvisorAzh#1{\gdef\@coadvisorAzh{#1}}

\def\coadvisorB#1{\gdef\@coadvisorB{#1}}

\def\coadvisorBzh#1{\gdef\@coadvisorBzh{#1}}

\def\authorzh#1{\gdef\@authorzh{#1}}

\def\watermark#1{\gdef\@watermark{#1}}

\def\acktitle#1{\gdef\@acktitle{#1}}

\def\toctitle#1{\gdef\@toctitle{#1}}

\def\loftitle#1{\gdef\@loftitle{#1}}

\def\lottitle#1{\gdef\@lottitle{#1}}

\def\bibtitle#1{\gdef\@bibtitle{#1}}

\def\cvtitle#1{\gdef\@cvtitle{#1}}

\def\loptitle#1{\gdef\@loptitle{#1}}

\def\reservedfrontpages#1{\gdef\@reservedfrontpages{#1}}


\ifTHESISOPTIONmaster
  \thesistype{Master Thesis}%
  \thesistypezh{碩士論文}%
  \degree{Master}%
  \reservedfrontpages{0}%
\else
  \thesistype{Doctoral Dissertation}%
  \thesistypezh{博士論文}%
  \degree{Doctor of Philosophy}%
  \reservedfrontpages{0}%
\fi

\ifTHESISOPTIONzh
  \acktitle{誌謝}%
  \toctitle{目錄}%
  \loftitle{圖目錄}%
  \lottitle{表目錄}%
  \bibtitle{參考文獻}%
  \cvtitle{自傳}%
  \loptitle{著作目錄}%
\else
  \acktitle{Acknowledgement}%
  \toctitle{Table of Contents}%
  \loftitle{List of Figures}%
  \lottitle{List of Tables}%
  \ifTHESISOPTIONmaster
    \bibtitle{References}%
  \else
    \bibtitle{Bibliography}%
  \fi
  \cvtitle{Curriculum Vitae}%
  \loptitle{List of Publications}%
\fi


\renewcommand{\cfttoctitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftaftertoctitle}{\hspace*{\fill}}
\renewcommand{\cftlottitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftafterlottitle}{\hspace*{\fill}}
\renewcommand{\cftloftitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftafterloftitle}{\hspace*{\fill}}

\ifTHESISOPTIONzh
  \renewcommand{\contentsname}{\makebox[3em][s]{\@toctitle}}%
  \renewcommand{\listfigurename}{\makebox[4em][s]{\@loftitle}}%
  \renewcommand{\listtablename}{\makebox[4em][s]{\@lottitle}}%
  \renewcommand{\tablename}{表}%
  \renewcommand{\figurename}{圖}%
\else
  \renewcommand{\contentsname}{\@toctitle}%
  \renewcommand{\listfigurename}{\@loftitle}%
  \renewcommand{\listtablename}{\@lottitle}%
\fi

\ifTHESISOPTIONzh
  \titlecontents{chapter}[0pt]{}%
  {\bfseries\xCJKnumber{\thecontentslabel}、\hspace{0.5em}}{}%
  {\cftdotfill{\cftdotsep}\contentspage}%
\else
  \titlecontents{chapter}[0pt]{}%
  {\bfseries\makebox[1em][l]{\thecontentslabel}\hspace{0.25em}}{}%
  {\cftdotfill{\cftdotsep}\contentspage}%
\fi

\renewcommand\cftbeforetoctitleskip{-0.5cm}
\renewcommand\cftbeforeloftitleskip{-0.5cm}
\renewcommand\cftbeforelottitleskip{-0.5cm}

\def\maketocs{%
\ifTHESISOPTIONreview\else
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@toctitle}}%
  \tableofcontents
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@loftitle}}%
  \listoffigures
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@lottitle}}%
  \listoftables
\fi
}


\ifTHESISOPTIONzh
  \titleformat{\chapter}[block]%
  {\centering\Huge\bfseries}%
  {\xCJKnumber{\thechapter}、\hspace{0.5em}}%
  {0em}{}%
\else
  \titleformat{\chapter}[display]%
  {\centering\Huge\bfseries}%
  {\chaptertitlename\ \thechapter}%
  {0em}{}%
\fi

\titlespacing*{\chapter}{0em}{-40pt}{*6}


\newcommand\BackgroundPicture{%
\ifTHESISOPTIONwatermark
  \ifTHESISOPTIONdraft
    \setlength{\@tempdimb}{.5\paperwidth}%
    \setlength{\@tempdimc}{.5\paperheight}%
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\@tempdimb,\strip@pt\@tempdimc){%
    \makebox(0,0){\rotatebox{45}{\textcolor[gray]{0.75}%
      {\fontsize{6cm}{6cm}\selectfont{DRAFT}}}}%
    }%
  \fi
  \ifTHESISOPTIONfinal
    \begin{tikzpicture}%
      \node[minimum width=\paperwidth,minimum height=\paperheight,opacity=0.75]%
        {\includegraphics[width=0.4\textwidth]{\@watermark}};%
    \end{tikzpicture}%
  \fi
\fi
}

\let\oldcleardoublepage\cleardoublepage
\renewcommand{\cleardoublepage}{%
  \newpage
  \ClearShipoutPicture
  \oldcleardoublepage
  \AddToShipoutPicture{\BackgroundPicture}%
}


\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 

\DeclareRobustCommand{\xCJKalphatozhnum}[1]{%
  \ifnum\strcmp{#1}{A} = 0 一 \else
  \ifnum\strcmp{#1}{B} = 0 二 \else
  \ifnum\strcmp{#1}{C} = 0 三 \else
  \ifnum\strcmp{#1}{D} = 0 四 \else
  \ifnum\strcmp{#1}{E} = 0 五 \else
  \ifnum\strcmp{#1}{F} = 0 六 \else
  \ifnum\strcmp{#1}{G} = 0 七 \else
  \ifnum\strcmp{#1}{H} = 0 八 \else
  \ifnum\strcmp{#1}{I} = 0 九 \else
  \ifnum\strcmp{#1}{J} = 0 十 \else
  \ifnum\strcmp{#1}{K} = 0 十一 \else
  \ifnum\strcmp{#1}{L} = 0 十二 \else
  \ifnum\strcmp{#1}{M} = 0 十三 \else
  \ifnum\strcmp{#1}{N} = 0 十四 \else
  \ifnum\strcmp{#1}{O} = 0 十五 \else
  \ifnum\strcmp{#1}{P} = 0 十六 \else
  \ifnum\strcmp{#1}{Q} = 0 十七 \else
  \ifnum\strcmp{#1}{R} = 0 十八 \else
  \ifnum\strcmp{#1}{S} = 0 十九 \else
  \ifnum\strcmp{#1}{T} = 0 二十 \else 零%
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}


\newcommand{\addBibToContents}{%
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@bibtitle}}%
}

\renewcommand{\bibname}{\makebox[5.5em][s]{\@bibtitle}}


\renewcommand{\thealgorithm}{\arabic{chapter}.\arabic{algorithm}}


\newcommand{\addAppxToContents}{%
\addtocontents{toc}{\protect\setcounter{tocdepth}{0}}
\ifTHESISOPTIONzh
  \titlecontents{chapter}[0pt]{}%
  {\bfseries 附錄\xCJKalphatozhnum{\thecontentslabel}\quad}%
  {}{\cftdotfill{\cftdotsep}\contentspage}%

  \titleformat{\chapter}[block]%
  {\centering\Huge\bfseries}%
  {附錄\xCJKalphatozhnum{\thechapter}\quad}%
  {0em}{}%
\else
  \titlecontents{chapter}[0pt]{}%
  {\bfseries \appendixname\hspace{0.5em}\thecontentslabel\hspace{0.5em}}%
  {}{\cftdotfill{\cftdotsep}\contentspage}%
\fi
}


\renewcommand\thesubfigure{ (\alph{subfigure})}


\def\coverpage
{
  \thispagestyle{empty}%
  \begin{center}
    \fontsize{18}{27}{\@universityzh}\\
    \fontsize{18}{27}{\@institutezh}\\
    \fontsize{18}{27}{\@thesistypezh}\\
    \ifTHESISOPTIONdraft
      \fontsize{18}{27}{初稿}\\
    \fi
    \vspace{2\baselineskip}
    
    \fontsize{14}{21}{\@institute}\\
    \fontsize{16}{24}{\@university}\\
    \fontsize{16}{24}{\@thesistype}\\
    \vspace{3\baselineskip} %

    \fontsize{18}{27}{\@titlezh}\\
    \vspace{0.75\baselineskip}
    \fontsize{18}{27}{\@title}\\
    \vspace{3\baselineskip} %
  
    \singlespacing
    \fontsize{18}{27}
    \begin{center}
    \begin{tabular}{c}%
      {研究生\ :} {\@authorzh \ (\@author)} \vspace{1em}\\%
      {指導教授\ :}{\@advisorzh \ (\@advisor)} \vspace{1em}\\%
      \ifx \@coadvisorAzh \@empty \else
        {\@coadvisorAzh(\@coadvisorA)} \vspace{1em}\\%
      \fi
      \ifx \@coadvisorBzh \@empty \else
        {\@coadvisorBzh(\@coadvisorB)} \vspace{1em}\\%
      \fi
    \end{tabular}%
    \end{center}
  \vspace{3cm}
  
  \fontsize{18}{27}\Large{\@nation} \Large{\@yearmonth}\\
  \LARGE{\@degreemonth} \ \LARGE{\@degreeyear} \\
  \end{center}
}


\def\titlepage
{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \begin{center}
    \singlespacing\Large
    \@titlezh\\
    \vspace{0.25\baselineskip}
    \@title\\
    \vspace{0.25\baselineskip}
  \end{center}
  \begin{flushleft}
    \singlespacing
    \setlength{\tabcolsep}{0.25em}
    \begin{tabular}{rl}%
      \large{\makebox[4em][s]{研究生}：}&\large{\@authorzh}\vspace{0.1em}\\%
      \large{指導教授：}&{\large{\@advisorzh}}\\%
      \ifx \@coadvisorAzh \@empty \else
        &{\large{\@coadvisorAzh}}\\%
      \fi
      \ifx \@coadvisorBzh \@empty \else
        &{\large{\@coadvisorBzh}}\\%
      \fi
    \end{tabular}%
    \hfill
    \begin{tabular}{ll}%
      \large{Student:}&{\large{\@author}}\vspace{0.5em}\\%
      \large{Advisor:}&{Dr. \large{\@advisor}}\\%
      \ifx \@coadvisorA \@empty \else
        &{\large{\@coadvisorA}}\\%
      \fi
      \ifx \@coadvisorB \@empty \else
        &{\large{\@coadvisorB}}\\%
      \fi
    \end{tabular}
  \end{flushleft}
  \vfill
  \begin{center}
    \large\@universityzh \vspace{-0.5em}\\
    \large\@institutezh \vspace{-0.5em}\\
    \ifTHESISOPTIONdraft
      \large\@thesistypezh \ 初稿\\
    \else
      \large\@thesistypezh\\
    \fi
    \vfill
    \ifTHESISOPTIONdraft
      \centerline{{A Thesis Draft}} \vspace{-1.0em}%
    \else
      \centerline{{A Thesis}} \vspace{-1.0em}%
    \fi
    Submitted to {\@institute} \vspace{-1.0em}\\
    \@college \vspace{-1.0em}\\
    \@university \vspace{-1.0em}\\
    in partial Fulfilment of the Requirements \vspace{-1.0em}\\
    for the Degree of \vspace{-1.0em}\\
    \@degree \vspace{-1.0em}\\
    in \vspace{-1.0em}\\
    \@field \vspace{-1.0em} \\
    \vspace{\baselineskip}
    \vfill
    {{\@degreemonth} {\@degreeyear}}\\
    \@location\\
    \vfill
    \Large{\@nation} \Large{\@yearmonth}
  \end{center}
}


\def\authzpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\approvalzhpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\approvalenpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\copyrightpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \rule[0pt]{0pt}{0pt} \\
  \vspace{2.5in}
  \rule[0pt]{0pt}{0pt} \\
  \begin{center}
    \copyright {\@degreeyear} - {\@author}\\
    \vspace{0.5\baselineskip}
    All rights reserved.\\
  \end{center}
}


\def\maketitle{{
\ifTHESISOPTIONreview\else
  \coverpage


  \titlepage
  
  \input{ack/ack}
  

  \frontmatter
  


\fi
}}


\def\abszhpage
{
  \cleardoublepage
  \ifTHESISOPTIONfinal
    \setcounter{page}{\the\numexpr\@reservedfrontpages+\arabic{page}\relax}
  \fi
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{摘要}}
  \begin{center}
    \singlespacing
    {\Large \bf \@titlezh}\\
    \vspace{\baselineskip}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{學生：}&{\large{\@authorzh}}\\%
      \end{tabular}&%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rlc}%
        \large{指導教授：}&{\large{\@advisorzh}}&{\large{博士}}\\%
        \ifx \@coadvisorAzh \@empty \else
          &{\large{\@coadvisorAzh}}&{\large{博士}}\\%
        \fi
        \ifx \@coadvisorBzh \@empty \else
          &{\large{\@coadvisorBzh}}&{\large{博士}}\\%
        \fi
      \end{tabular}\\%
    \end{tabular*}\\
    \vspace{0.5\baselineskip}
    \large{\@universityzh\hspace{1ex}\@institutezh}\\
    \vspace{\baselineskip}
    \Large{\textbf{摘\qquad 要}}\\
  \end{center}
}

\newenvironment{abstractzh}{%
  \ifTHESISOPTIONreview\else
    \abszhpage
    \par %
  \fi
  \ifTHESISOPTIONreview\comment\fi  %
}{%
  \ifTHESISOPTIONreview\endcomment\fi
}


\def\absenpage
{
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{Abstract}}
  \begin{center}
    \singlespacing
    {\Large \bf \@title}\\
    \vspace{\baselineskip}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{Student:}&{\large{\@author}}\\%
      \end{tabular}&%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{Advisor:}&{\large{Dr. \@advisor}}\\%
        \ifx \@coadvisorA \@empty \else
          &{\large{Dr. \@coadvisorA}}\\%
        \fi
        \ifx \@coadvisorB \@empty \else
          &{\large{Dr. \@coadvisorB}}\\%
        \fi
      \end{tabular}\\%
    \end{tabular*}\\
    \vspace{0.5\baselineskip}
    \large{\@institute}\\
    \large{\@university}\\
    \vspace{\baselineskip}
    \Large{\textbf{Abstract}}\\
  \end{center}
}

\newenvironment{abstract}{%
  \ifTHESISOPTIONreview\else
    \absenpage
    \par %
  \fi
  \ifTHESISOPTIONreview\comment\fi  %
}{%
  \ifTHESISOPTIONreview\endcomment\fi
}


\def\ackpage
{
  \cleardoublepage
  \ClearShipoutPicture  %
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@acktitle}}
  \begin{center}
    \ifTHESISOPTIONzh
      {\LARGE \bf \makebox[3em][s]{\@acktitle}}\\
    \else
      {\LARGE \bf \@acktitle}\\
    \fi
  \end{center}
}

\newenvironment{acknowledgement}{%
  \ifTHESISOPTIONfinal
    \ackpage
    \par %
  \fi
  \ifTHESISOPTIONfinal\else\comment\fi  %
}{%
  \ifTHESISOPTIONfinal\else\endcomment\fi
}


\newenvironment{dedication}{%
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd
    \cleardoublepage
    \ClearShipoutPicture  %
    \thispagestyle{empty}%
    \vspace*{6.6cm}
    \begin{center}
  \fi\fi
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd\else\comment\fi\else\comment\fi
}{%
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd\else\endcomment\fi\else\endcomment\fi
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd
    \end{center}
  \fi\fi
}


\newenvironment{vita}{%
  \ifTHESISOPTIONreview\comment\else\ifTHESISOPTIONphd\else\comment\fi\fi
    \cleardoublepage
    \phantomsection
    \addcontentsline{toc}{chapter}{\textbf{\@cvtitle}}
    \ifTHESISOPTIONzh
      \chapter*{\makebox[3em][s]{\@cvtitle}}
    \else
      \chapter*{\@cvtitle}
    \fi
}{%
  \ifTHESISOPTIONreview\endcomment\else\ifTHESISOPTIONphd\else\endcomment\fi\fi
}


\newenvironment{publications}{%
  \ifTHESISOPTIONreview\comment\else\ifTHESISOPTIONphd\else\comment\fi\fi
    \cleardoublepage
    \phantomsection
    \addcontentsline{toc}{chapter}{\textbf{\@loptitle}}
    \ifTHESISOPTIONzh
      \chapter*{\makebox[5.5em][s]{\@loptitle}}
    \else
      \chapter*{\@loptitle}
    \fi
}{%
  \ifTHESISOPTIONreview\endcomment\else\ifTHESISOPTIONphd\else\endcomment\fi\fi
}

\endinput

